From Network Traces to System Responses: Opaquely Emulating Software Services

Enterprise software systems make complex interactions with other services in their environment. Developing and testing for production-like conditions is therefore a challenging task. Prior approaches include emulations of the dependency services using either explicit modelling or record-and-replay approaches. Models require deep knowledge of the target services while record-and-replay is limited in accuracy. We present a new technique that improves the accuracy of record-and-replay approaches, without requiring prior knowledge of the services. The approach uses multiple sequence alignment to derive message prototypes from recorded system interactions and a scheme to match incoming request messages against message prototypes to generate response messages. We introduce a modified Needleman-Wunsch algorithm for distance calculation during message matching, wildcards in message prototypes for high variability sections, and entropy-based weightings in distance calculations for increased accuracy. Combined, our new approach has shown greater than 99% accuracy for four evaluated enterprise system messaging protocols.

==> introduction_old.tex <==
\section{Introduction}
% no \IEEEPARstart

Aims:
Automatic method for service emulation derived from message trace

Opaqueness: don't assume any knowledge of the message structure

High Accuracy

Real-time performance

Robust

Contributions:

Method for automatic generated message prototypes
\begin{itemize}
    \item Application of multiple sequence alignment algorithm to derive message prototypes
    \item Introduction of wildcards for high variability sections of messages
    \item Use of modified Needleman-Wunsch for message distance calculations
    \item Application of entropy weighting in distance calculations for increased accuracy
\end{itemize}

Method for automatically separating the payload and structure information (for discussion: improves robustness)

Aim is generate responses (not models)

Generate real responses - not just a model - going a different path (go further without an explicit model)

$>99\%$ accuracy for 6 protocols tested

Background and Motivation:

With the trend of every increasing inter-connectedness between software systems, service emulation is needed to develop and test a software system, independent of the other systems on which it depends.

Emphasis on service emulation (not client emulation).

Previous approaches to service emulation have relied on explicit modelling by a system expert or knowledge of message protocols and structure.  This is not always available.

Our aim is to develop an automated approach to service emulation which uses no explicit knowledge of message protocols and structure.

Our previous work proposed searching message traces to automatically generate responses.  Was limited to text based protocols and became inefficient for large message traces.  Method was sensitive to mismatching by payload versus operation type (not robust.)  Subsequent work used clustering to improve efficiency by decreased accuracy.  The aim of this work is to achieve both higher accuracy and efficiency through descriptive and robust message prototypes which can be applied to both binary and text protocols.


==> timing.tex <==
% Document Type: LaTeX
% Master File: timing.tex
% Author: Jean-Guy Schneider
% Last Modified: Fri Sep 5 2014, 14:32

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\resgentime}{
    \begin{tabular}{|>{\centering\arraybackslash}m{0.8cm} |c|>{\centering\arraybackslash}m{1.1cm} |>{\centering\arraybackslash}m{1.1cm} |>{\centering\arraybackslash}m{1.5cm} |>{\centering\arraybackslash}m{1cm}|}
        \hline
      % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
       &No.& Whole Library  & Cluster Centroid & Consensus +Weighting & Real System \\\hline\hline
      IMS  &800& 432 & 4.39 & 2.86 & 518 \\ \hline
      LDAP &2177& 781 & 2.11 & 2.23 & 28  \\ \hline
      LDAP text(1) &2177 & 1176.1 & 5.64 & 6.83 & 28 \\ \hline
      LDAP text(2) &1000& 91.29 & 1.40 & 1.31 & 28 \\ \hline
      SOAP &1000& 328.79 & 2.90 & 3.07 & \\ \hline
      Twitter&1825& 419.82 & 48.84 & 49.45 & 417 \\ \hline
    \end{tabular}
}
\newcommand{\matchingtime}{
 \resizebox{0.49\textwidth}{!}{
    \begin{tabular}{|>{\centering\arraybackslash}m{0.8cm} |c|>{\centering\arraybackslash}m{0.8cm} |>{\centering\arraybackslash}m{0.6cm} |>{\centering\arraybackslash}m{0.6cm} 
    |>{\centering\arraybackslash}m{0.6cm} |>{\centering\arraybackslash}m{0.6cm} |>{\centering\arraybackslash}m{0.6cm} |}
  
   % \begin{tabular}{|c|c|c|c|c|c|c|c|}
        \hline
      % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
       \multirow{2}{0.5cm}{}&\multirow{2}{0.5cm}{\centering No.}& \multicolumn{2}{c|}{\multirow{1}{*}{Whole Library}}  & \multicolumn{2}{c|}{\multirow{1}{*}{Cluster Centroid}} & \multicolumn{2}{c|}{Consensus+W} \\\cline{3-8}
       &&M&S&M&S&M&S \\\hline\hline
      \multirow{1}{0.5cm}{IMS} &800& 431.43 & 0.41 & 3.35 & 0.98 & 2.31 & 0.61 \\ \hline
      LDAP &2177& 771.54 & 6.28 & 1.58 & 0.27 & 2.03 & 0.21 \\ \hline
      LDAP text(1) &2177 & 1174.81 & 1.18 & 4.31 & 1.17 & 5.37 & 1.33 \\ \hline
      LDAP text(2) &1000& 91.17 & 4.18 & 0.77 & 0.64 & 0.96 & 0.35 \\ \hline
      SOAP &1000& 330.38 & 1.19 & 1.88 & 0.97  & 2.16 & 0.87 \\ \hline
      Twitter &1825& 352.65 & 51.11& 0.86 & 48.03 & 1.23 & 48.29 \\ \hline
    \end{tabular}
 }   
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% Original Tables %%%%

% \newcommand{\resgentime}{
%     \begin{tabular}{|>{\centering\arraybackslash}m{0.8cm} |c|>{\centering\arraybackslash}m{1.1cm} |>{\centering\arraybackslash}m{1.1cm} |>{\centering\arraybackslash}m{1.5cm} |>{\centering\arraybackslash}m{1cm}|}
%         \hline
%       % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
%        &No.& Whole Library  & Cluster Centroid & Consensus +Weighting & Real System \\\hline\hline
%       IMS  &800& 470.99 & 4.94 & 3.24& 518\\ \hline
%       LDAP &2177& 835.91 & 2.77 & 2.88 & 28  \\ \hline
%       LDAP text(1) &2177 & 1434.70 & 5.69 & 7.30 & 28 \\ \hline
%       LDAP text(2) &1000& 266.30 & 2.44 & 1.63 & 28 \\ \hline
%       SOAP &1000& 380.24 & 2.97 & 3.35 & \\ \hline
%       Twitter&1825& 464.09 & 32.86 & 36.62 & 417 \\ \hline
%     \end{tabular}
% }
% \newcommand{\matchingtime}{
%  \resizebox{0.49\textwidth}{!}{
%     \begin{tabular}{|>{\centering\arraybackslash}m{0.8cm} |c|>{\centering\arraybackslash}m{0.8cm} |>{\centering\arraybackslash}m{0.6cm} |>{\centering\arraybackslash}m{0.6cm} 
%     |>{\centering\arraybackslash}m{0.6cm} |>{\centering\arraybackslash}m{0.6cm} |>{\centering\arraybackslash}m{0.6cm} |}
  
%    % \begin{tabular}{|c|c|c|c|c|c|c|c|}
%         \hline
%       % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
%        \multirow{2}{0.5cm}{}&\multirow{2}{0.5cm}{\centering No.}& \multicolumn{2}{c|}{\multirow{1}{*}{Whole Library}}  & \multicolumn{2}{c|}{\multirow{1}{*}{Cluster Centroid}} & \multicolumn{2}{c|}{Consensus+W} \\\cline{3-8}
%        &&M&S&M&S&M&S \\\hline\hline
%       \multirow{1}{0.5cm}{IMS} &800& 460.78&10.2 & 3.67 &1.27 & 2.68&0.56 \\ \hline
%       LDAP &2177& 828.95 & 6.96 & 2.38 &0.39& 2.60&0.28 \\ \hline
%       LDAP text(1) &2177 & 1425.23 &9.47& 4.38&1.31 & 5.67&1.63 \\ \hline
%       LDAP text(2) &1000& 257.92 &8.38& 1.35 &1.09& 1.14 &0.49\\ \hline
%       SOAP &1000& 372.58 &7.66& 1.92 &1.05 & 2.45 &0.9\\ \hline
%       Twitter &1825& 412.98 &51.11& 1.47 &31.39& 1.67 &34.95 \\ \hline
%     \end{tabular}
%  }   
% }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

